Robust Anytime Learning of Markov Decision Processes

Markov decision processes (MDPs) are formal models commonly used in sequential decision-making. MDPs capture the stochasticity that may arise, for instance, from imprecise actuators via probabilities in the transition function. However, in data-driven applications, deriving precise probabilities from (limited) data introduces statistical errors that may lead to unexpected or undesirable outcomes. Uncertain MDPs (uMDPs) do not require precise probabilities but instead use so-called uncertainty sets in the transitions, accounting for such limited data. Tools from the formal verification community efficiently compute robust policies that provably adhere to formal specifications, like safety constraints, under the worst-case instance in the uncertainty set. We continuously learn the transition probabilities of an MDP in a robust anytime-learning approach that combines a dedicated Bayesian inference scheme with the computation of robust policies. In particular, our method (1) approximates probabilities as intervals, (2) adapts to new data that may be inconsistent with an intermediate model, and (3) may be stopped at any time to compute a robust policy on the uMDP that faithfully captures the data so far. Furthermore, our method is capable of adapting to changes in the environment. We show the effectiveness of our approach and compare it to robust policies computed on uMDPs learned by the UCRL2 reinforcement learning algorithm in an experimental evaluation on several benchmarks.

==> sampling.tex <==
\section{Exploration Policies}\label{sec:sampling}
In this section, we discuss how to obtain the trajectories the previous section assumed given.
Aiming for acceptable sample efficiency, we make our exploration policies specification-driven by only sampling transitions along trajectories towards the target state(s) of the specification.
When the last seen state has probability zero or one to reach the target for reachability, or reward zero or infinity for reward specifications, we restart.
States satisfying these conditions can be found by analyzing the graph of the true MDP~\citep{DBLP:books/daglib/Baier2008}.





We define three exploration policies: 1) \emph{uniform} exploration, which is used as a baseline for comparison, 2) \emph{optimistic} exploration, and 3) \emph{reward-based} exploration. 


\begin{definition}[Exploration policies]\label{def:expl_policies}
Let $T$ be the set of target states of the specification $\spec$, and recall the notion of optimistic specifications from Sect.~\ref{sec:preliminaries}. We define the following exploration policies:
\begin{itemize}
    \item \emph{Uniform exploration}. We define the uniform exploration policy by taking the uniform distribution over the actions at every state:
	$
	\forall s \in S, a \in A.\,	\strat(s,a) = \frac{1}{|A|}.
	$
	\item \emph{Optimistic exploration. } We define the optimistic counterpart of the specification $\spec$, \ie $\spec_O$, and compute the optimal policy in the current uMDP for this specification.
	\item \emph{Reward-based exploration. } We define a reward function $R$ as the sum of the sizes of the intervals at a state-action pair, normalized by the number of successor states: 
	\begin{align}
	\forall s \in S. \forall a \in A. \,R(s,a) = \frac{\sum_{s' \in \succ(s,a)} |\utransfunc(s,a,s')|}{|\succ(s,a)|},
    \end{align}
	and then compute the optimal policy in the current uMDP for the optimistic specification \emph{$\Rmaxmax(\eventually T)$}.
\end{itemize}

\end{definition}

It should be noted that the optimistic and reward-based exploration policies are only possible to compute on a uMDP, since they rely on the intervals.










\noindent


\noindent

\paragraph{Trajectories and iterations. } As explained in Sect.~\ref{sec:problem}, our method is iterative in terms of updating the uMDP $\mathcal{M}$ and computing a robust policy. 
After updating the uMDP, we also compute a new optimistic or reward-based exploration policy, as those depend on the intermediate uMDP.
Each iteration consists of processing at least one, but possibly more trajectories.
To determine how many trajectories to collect, we use a doubling-counting scheme, where we keep track of how often every state-action pair and transition is visited during exploration~\citep{DBLP:conf/icml/JinJLSY20}.
An iteration is completed when any of the counters is doubled with respect to the previous iteration.
A detailed description of this schedule is given in Appx.~A.












